Observability Analysis of Aided INS with Heterogeneous Features of Points, Lines and Planes

In this paper, we perform a thorough observability analysis for linearized inertial navigation systems (INS) aided by exteroceptive range and/or bearing sensors (such as cameras, LiDAR and sonars) with different geometric features (points, lines and planes). While the observability of vision-aided INS (VINS) with point features has been extensively studied in the literature, we analytically show that the general aided INS with point features preserves the same observability property: that is, 4 unobservable directions, corresponding to the global yaw and the global position of the sensor platform. We further prove that there are at least 5 (and 7) unobservable directions for the linearized aided INS with a single line (and plane) feature; and, for the first time, analytically derive the unobservable subspace for the case of multiple lines/planes. Building upon this, we examine the system observability of the linearized aided INS with different combinations of points, lines and planes, and show that, in general, the system preserves at least 4 unobservable directions, while if global measurements are available, as expected, some unobservable directions diminish. In particular, when using plane features, we propose to use a minimal, closest point (CP) representation; and we also study in-depth the effects of 5 degenerate motions identified on observability. To numerically validate our analysis, we develop and evaluate both EKF-based visual-inertial SLAM and visual-inertial odometry (VIO) using heterogeneous geometric features in Monte Carlo simulations.

==> sections/apd.tex <==
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

==> sections/biography.tex <==
%!TEX root = ../main.tex

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yangyulin.jpg}}]{Yulin Yang}
received the B.Eng. degree in Mechanical Engineering from Shandong University, China, in 2009, and M.Sc. in Mechanical Engineering from Xi'an Jiaotong University, China in 2012. 
He is currently working toward a Ph.D. in department of Mechanical Engineering at University of Delaware. From 2012 to 2015, he was a Research \& Development Engineer at Siemens High Voltage Research Center in Shanghai, China. 


His research topics focus on visual inertial navigation, SLAM and nonlinear estimation. 
\end{IEEEbiography}




% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Huang2014small.jpg}}]{Guoquan Huang}
received the B.Eng. in automation (electrical engineering) from University of Science and Technology Beijing,  China,  in  2002,  and  the  M.Sc.  and  Ph.D. in computer science from University of Minnesota--Twin Cities, Minneapolis, MN, USA, in 2009 and 2012, respectively. 


He  is  currently an Assistant Professor of Mechanical Engineering (ME), Electrical and Computer Engineering (ECE), and Computer and Information Sciences (CIS), at the University of Delaware (UD), Newark, DE, USA, where he is leading the Robot Perception and Navigation Group (RPNG). He is also an Adjunct Professor at the Zhejiang University, Hangzhou, China and a Senior Consultant at the Huawei 2012 Laboratories. From 2012 to 2014, he was a Postdoctoral Associate at MIT Computer Science and Artificial Intelligence Laboratory (CSAIL), Cambridge, MA, USA.
 %
His research interests  include sensing, localization, mapping, and perception of autonomous ground, aerial, and underwater robots. 


Dr. Huang received the 2006 Academic Excellence Fellowship from the University of Minnesota, the 2011 Chinese Government Award for Outstanding Self-Financed Students Abroad, the 2013 MIT Postdoctoral Associate Travel Award, the 2015 UDRF Award, the 2016 NSF CRII Award, the 2017 UD Makerspace Faculty Fellow, 2018 SATEC robotics delegation,  and was the Finalist for the 2009 Best Paper Award from the Robotics: Science and Systems Conference (RSS).
\end{IEEEbiography}





% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:


% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
